On the Statistical Relation of Ultra-Reliable Wireless and Location Estimation

Location information is often used as a proxy to guarantee the performance of a wireless communication link. However, localization errors can result in a significant mismatch with the guarantees, particularly detrimental to users operating the ultra-reliable low-latency communication (URLLC) regime. This paper unveils the fundamental statistical relations between location estimation uncertainty and wireless link reliability, specifically in the context of rate selection for ultra-reliable communication. We start with a simple one-dimensional narrowband Rayleigh fading scenario and build towards a two-dimensional scenario in a rich scattering environment. The wireless link reliability is characterized by the meta-probability, the probability with respect to localization error of exceeding the outage capacity, and by removing other sources of errors in the system, we show that reliability is sensitive to localization errors. The $\epsilon$-outage coherence radius is defined and shown to provide valuable insight into the problem of location-based rate selection. However, it is generally challenging to guarantee reliability without accurate knowledge of the propagation environment. Finally, several rate-selection schemes are proposed, showcasing the problem's dynamics and revealing that properly accounting for the localization error is critical to ensure good performance in terms of reliability and achievable throughput.

==> sections/channel.tex <==
\subsection{Communication System and Channel Model} \label{subsec:chn_model}
A cellular network has several \glspl{bs} installed in an area, and can be used for both localization and data transmission. The considered scenario is a 2-D framework and this section characterizes the channel between one of the \glspl{bs} at location $\mbf{x}_{\text{bs}} \in \mR^2$ and a \gls{ue} at location $\mbf{x} \in \mR^2$. Both the \gls{bs} and the user are equipped with a single antenna and an \gls{ofdm} modulation scheme is considered, with bandwidth $W$ and $N$ subcarriers spaced $\Delta_f = W/N$. 

The channel between the \gls{ue} and the \gls{bs} is modeled according to some simple (stochastic) models for the channel coefficients and their respective delays, which enables us statistically analyze the system based on a few parameters while also simulating a realistic scenario. \TK{Put some more motivation for the approach in the introduction}
The modeled channel has an $K$ number of paths with complex channel coefficients $a_{k}$ and associated delays $\tau_{k}$ for paths $k = 1, \dots, K$. With \gls{ofdm} modulation and symbol $\mbf{s} \in \mC^N$, the received baseband signal in the frequency domain across the different subcarriers, $\tilde{\mbf{y}} \in \mC^N$, is then given by\footnote{We assume identical uplink and downlink channels.} \cite{wymeersch_beyond_2020}
\begin{align} \label{eq:sysmod}
\tilde{y}_{j} =\sqrt{P_{\text{tx}}}\sum_{k=1}^{K}a_k d_j(\tau_k) s_j + \tilde{n}_{j},\quad  j = 0,\dots, N - 1,
\end{align}
where $P_{\text{tx}}$ is the transmit power per subcarrier, $\tilde{n}_{j}\sim \mathcal{CN}(0, \sigma_n^2)$ is the noise term with variance $\sigma_n^2$, and $d_j(\tau) = \exp\left(-\jmath\pi2j\Delta_f \tau\right)$. In the channel model \eqref{eq:sysmod}, the first path ($k=1$) is the deterministic \gls{los} path while the remaining paths ($1 < k \leq K$) are the contributions from different scatters modeled stochastically. The two types of paths are described separately. 
\subsubsection{LoS path}
The \gls{los} path characterizes the attenuation of the signal as a function of distance between the \gls{bs} and the \gls{ue}. It comprises 3 parts: path loss $P_L$, shadowing $\psi$, and phase rotation $\phi$, and is given by\cite{tse_vis,wymeersch_beyond_2020}
\begin{align}
a_{1}(\mbf{x}) = \sqrt{P_L(d)\psi(\mbf{x})} \e^{-\jmath\phi(d)},   
\end{align}
where $d = \norm{\mbf{x}_{\text{bs}} - \mbf{x}}$ is the distance to the \gls{bs}, and $\lambda$ is the wavelength, and the phase rotation is $\phi(d) = 2\pi d/\lambda$. Naturally, it follows that the \gls{los} delay $\tau_1$  is $d/c $ with $c$ the speed of light. Path loss is modeled according to the log-distance path-loss model\cite{goldsmith2005wireless}
\begin{align}
    P_L(d) \ [\text{dB}] = G_0 - 10\eta\log_{10}\left(\frac{d}{d_0}\right),
\end{align}
where $G_0$ is the constant gain in dB at reference distance $d_0$ and $\eta$ is the path loss exponent. The shadowing component $\psi$ models the slow variations in space produced by large obstacles like trees or buildings. It is modeled statistically according to a log-normal shadowing model which assumes that $\psi_{\text{dB}} = 10\log_{10}(\psi)$ follows a normal distribution with zero mean and spatial correlation according to the Gudmundson correlation model, which has been experimentally verified and is often used in the literature to model shadowing \cite{Gudmundson1991}. This model assumes that the shadow fading is spatially correlated such that $\psi_{\text{dB}}$ is a zero mean Gaussian process, where the correlation of shadow fading between two users at locations $\mbf{x}_1$ and $\mbf{x}_2$ is given by
\begin{align}
    C_{\psi}(\mbf{x}_1,\mbf{x}_2) = \Cov\left[\psi_{\text{dB}}(\mbf{x}_1), \psi_{\text{dB}}(\mbf{x}_2)\right] = \sigma_{\psi}^2\exp\left(-\frac{   \norm{\mbf{x}_1-\mbf{x}_2}}{d_c}\right), \label{eq:Gudmundson}
\end{align}
where $\sigma_{\psi}^2$ is the shadowing variance, and $d_c > 0$ is the correlation distance, which tends to be in order of the size of the blocking objects in the environment \cite[ch. 2]{goldsmith2005wireless}. Note that, due to the logarithmic transformation, the expected value of the shadowing is different from one, i.e.,  \TK{Working in the natural logarithmic domain would remove the scalars. We can remove this comment later on. }
\begin{align}
    E[\psi(\mbf{x})] = \exp\left(E\left[\frac{\ln(10)}{10}\psi_{\text{dB}}(\mbf{x})\right] + \frac{1}{2}\Var\left[\frac{\ln(10)}{10}\psi_{\text{dB}}(\mbf{x})\right]\right) = \exp\left(\frac{\ln^2(10)}{200}\sigma_{\psi}^2 \right) \neq 1.
\end{align}
However, the median value of $\psi$ is $1$. 

\subsubsection{Scattered paths}
The remaining paths  ($1 < k \leq K$) represent the contribution from  scattered paths. They are modeled as proportional to the first path with an additional fast fading coefficient $\alpha$ depending on the delay, hence $a_k = \sqrt{P_L(d)\psi(\mbf{x})}\alpha_k(\tau_k)$. The fast fading coefficient arises from a number scatter of paths that cannot be mutually resolved at the receiver giving rise to the model $\alpha_{k}\sim\mathcal{CN}(0, \sigma^2(\tau_k))$ \cite[ch. 3]{goldsmith2005wireless}. Furthermore, the variance $\sigma^2(\tau_k)$ of is assumed to follow an exponential power delay profile as a function of the delay \cite{krouk} with parameters $A_{\text{SCAT}}$ and $\rho$, i.e., 
\begin{align} 
\sigma^2(\tau_k) = \Var[\alpha_{k}] =A_{\text{SCAT}}\exp\left(- \frac{\tau_k - \tau_1}{\rho} \right). \label{eq:scatter_stats}
\end{align}
The parameter $A_{\text{SCAT}} \in (0,1]$ is the attenuation factor of a scattered path versus the \gls{los} path (if they had the same delay), hence,  $E[|a_k(\tau_1)|^2] = A_{\text{SCAT}}|a_1|^2$ for $k> 1$. The parameter $\rho$ controls how fast the power fades as a function of the delay and is chosen such that a difference in delay of $1/W$ will scale the variance with a factor of $P_{\text{SCAT}} \in (0,1)$, i.e.,
\begin{align}
    \sigma^2\left(\tau_k + \frac{1}{W}\right) = P_{\text{SCAT}}\sigma^2(\tau_k) \Leftrightarrow  \rho = -\frac{1}{W\ln(P_{\text{SCAT}})}
\end{align}
Note that the choice to model $\alpha_{k}$ statistically, unlike, e.g., the deterministic geometric models in~\cite{wymeersch_beyond_2020}, is made to allow for statistical analysis of the communication reliability. 

It remains to model the delays $\tau_k$ for $1 < k \leq  K$, which will also be done statistically. A common assumption for this is to assume a Poisson process, where the excess delays ${\Delta\tau_k = \tau_{k+1} - \tau_{k}}$ for $k = 1,\dots, K-1$ are independent and identically distributed following the exponential distribution \cite{krouk}. However, to enforce spatial consistency in the modeled 2D scenario, we will assume a multivariate exponential distribution for each scatter $k$. For this, define the stochastic process over $\mathbb{R}^2$ as
\begin{align}
\Delta\mathcal{T}_k = \left\{\Delta T_k(\mbf{x}) : x \in \mR^2 \right\},
\end{align}
where $\Delta T_k(\mbf{x})$ is excess delay for path $k$ with respect to path $k-1$ at location $\mbf{x}$. For a finite subset of $d$ locations $\mbf{X} = \begin{bmatrix}\mbf{x}_1^\T & \dots \mbf{x}_d^\T \end{bmatrix}^\T \in \mathbb{R}^{2 \times d}$, we denote the excess delay vector for those points as  $\Delta \mbf{T}_k(\mbf{X}) \in \mR^d$. In a practical scenario, the experienced delay for a given path should (at least locally) vary smoothly in space following the geometry of the environment. Hence, we assume a multivariate exponential distribution generated from correlated Gaussian variables that was introduced in \cite{Mallik2003}. The distribution is generated in the following way. First, assume that the variables $\mbf{R}_k' \in \mR^d$ and $\mbf{R}_k'' \in \mR^d$ are IID multivariate Gaussian variables with zero mean and covariance $\frac{1}{2}\mbs{\Sigma}_R$. The excess delay is then generated as ${\Delta T_k(\mbf{x}_i) = (R_k')_i^2 + (R_k'')_i^2}$ for $i = 1,\dots, d$, and $\Delta \mbf{T}_k(\mbf{X})$ becomes a multivariate exponential distribution whose marginal distributions are exponential\cite{Mallik2003}. To ensure a smooth variation of the excess delays, we assume an exponential correlation matrix
\begin{align}
    (\mbf{\Sigma}_R)_{ij} = \overline{\tau}e^{-\norm{\mbf{x}_i - \mbf{x}_j}^2/d_{\tau}}, \label{eq:delay_cov}
\end{align}
with parameters $\overline{\tau}, d_{\tau} > 0$ similar to the Gudmundson correlation model with the notable exception of the squared norm. It follows from \eqref{eq:delay_cov} that\cite{Mallik2003}:
\begin{align}
    E[\Delta T_k(\mbf{x}_i)] &= \overline{\tau} \\
    \Var[\Delta T_k(\mbf{x}_i)] &= \overline{\tau}^2 \\
    \Cov[\Delta T_k(\mbf{x}_i), \Delta T_k(\mbf{x}_j)] &= \overline{\tau}^2e^{-2\norm{\mbf{x}_i - \mbf{x}_j}^2/d_{\tau}} 
\end{align}
Thus, $\overline{\tau}$ is the mean excess delay and $d_\tau$ controls how fast the correlation of delays fades as a function of distance. Moreover, the marginal excess delay distribution of the paths $k = 1,\dots, K - 1$ are exponential with mean $\overline{\tau}$ and it is easily shown that the average delay for path $k$ fulfills  $E[\tau_k] = \tau_1 + (k-1)\overline{\tau}$. \TK{$\tau_k - \tau_1$ is gamma distributed with shape $k-1$ and scale $\overline{\tau}$}
\\[\baselineskip]
In summary, the channel model comprises path loss, shadowing and fast fading. The first path is the deterministic \gls{los} path affected by only path loss and shadowing while the remaining $K - 1$ paths are also affected by fast fading whose variance depends on the delays for each scatter. The propagation environment is assumed to be stationary meaning that for any scenario, the shadowing $\psi(\mbf{x})$ and excess delay distribution $\Delta T_k(\mbf{x})$ for $k \geq 1$ stays constant and only the fast fading coefficient $\alpha_k$ varies over time. 

\subsection{Localization and Communication Protocol}

The following simple two-step protocol is assumed:
\begin{enumerate}
    \item  When the \gls{ue} turns on for the first time, it estimates its location using a ping --- a single \gls{ofdm} symbol as in \eqref{eq:sysmod} with $s_j = 1$ $\forall$ $j$ --- from each \gls{bs}. To that end, \gls{toa} estimation is employed. Moreover, the pings are used to select the \gls{bs} with which the \gls{ue} will communicate based on the received power, i.e., \gls{bs} $i \in \{1,2\}$ is chosen such that $\|\mbf{\widetilde{y}}_i\|^2$ is maximized. 
\item Once the \gls{ue} has estimated its location and the target \gls{bs}, it starts the communication with the chosen \gls{bs} by sending data (power normalized $E[|s_j|^2]=1$) using the OFDM channel with rate $R$. It is assumed that the channels used in steps 1 and 2 are independent. 
\end{enumerate}


To inform rate selection, we introduce the \gls{mar} $R_{\max}$ \TK{can we call it capacity?} as an information-theoretic bound, and the \gls{ue} should select $R$ such that it only exceeds $R_{\max}$ with low probability (explained further in Sec. X). Following the Sec. \ref{sec:intro}, it is assumed that a mapping between location $x$ and the statistics of $R_{\max}$ is available to the \gls{ue}. We then analyze how localization errors affect the reliability and throughput of the system when the \gls{ue} selects $R$ using different location-based rate selection schemes.

% \section{Statistical analysis of the subcarriers}
% To analyze the mode, we characterize the power of the subcarriers statistically. We first assume block fading, where the channel is drawn independently between each block (possibly extending multiple \gls{ofdm} symbols). We also assume that the propagation environment is stationary in the sense that only the second path changes in time due to small-scale fading. From this it follows that the first path $a_1$ only depends on location whereas the second path $a_2$ both depends on both location and time, i.e,
% \begin{align}
%     \tilde{h}_j(\mbf{x},t) = a_{1}(\mbf{x})d_j(\tau_{1}) + a_{2}(\mbf{x},t)d_j(\tau_{2}),
% \end{align}
% where $t$ denotes the block index. The dependency on time and location is separated by the following derivations. Omitting the explicit dependence on $\mbf{x}$ and $t$, the steering vector for the first path is factored out
% \begin{align}
%     \tilde{h}_j = a_{1}d_j(\tau_{1}) + a_{2}d_j(\tau_{2}) = d_j(\tau_{1})\left(a_{1} + a_{2}d_j(\Delta\tau)\right)
% \end{align}
% Defining $\tilde{a}_2 = a_2/\sqrt{P_L(d)\psi(\mbf{x})}$, it follows that
% \begin{align}
%     \tilde{a}_2 \sim \mathcal{CN}\left(0,\frac{1}{\rho}\exp\left(- \frac{\Delta\tau}{\rho} \right)\right)
% \end{align}
% does not depend on the location. The power of the subcarrier is then written
% \begin{align}
%     P = |\tilde{h}_j|^2 &= |d_j(\tau_1)|^2|\sqrt{P_L(d)\psi(\mbf{x})} \e^{-\jmath\phi(d)} + \sqrt{P_L(d)\psi(\mbf{x})}\tilde{a}_2 d_j(\Delta\tau) |^2 \\
%     &= P_L(d)\psi(\mbf{x})|\underbrace{\e^{-\jmath\phi(d)}  + \tilde{a}_2 d_j(\Delta\tau)}_{\check{a}}|^2 
% \end{align}
% By noting that 
% \begin{align}
%     |E[\check{a}]|^2 &= |\e^{-\jmath\phi(d)}|^2 = 1 \\
%     \Var[\check{a}] &= |d_j(\Delta\tau)|^2\Var[\tilde{a}_2] = \Var[\tilde{a}_2],
% \end{align}
% it follows that $\alpha = |\check{a}|^2$ is Rician distributed with parameters
% \begin{align}
%     A &= E[\alpha] = E[|\check{a}|^2] = E[\check{a}]|^2 + \Var[\check{a}] = 1 + \frac{1}{\rho}\exp\left(- \frac{\Delta\tau}{\rho} \right) \\
%     K &= \frac{|E[\check{a}]|^2}{\Var[\check{a}]} = \rho\exp\left(\frac{\Delta\tau}{\rho} \right),
% \end{align}
% where $A$ is the average power and $K$ is the Rician k-factor. 
% The power of the subcarrier is then $P =  P_L(d)\psi(\mbf{x})\alpha$, where 
% \begin{itemize}
%     \item $P_L(d)$ is deterministic and only depends on the distance between the \gls{ue} and the \gls{bs}
%     \item $\psi(\mbf{x})$ is spatially correlated and depends on the location of the \gls{ue}. The spatial correlation is given by the Gudmundson correlation model \eqref{eq:Gudmundson} and $\psi(\mbf{x})$ is modeled as a zero-mean Gaussian process in the logarithmic domain. 
%     \item $\alpha$ does not depend on the location and only changes with the block. 
% \end{itemize}
% Interestingly, the statistics of the received power does not depend on the subcarrier index. However, since each subcarrier is simply a different linear combination of $a_1$ and $a_2$, all subcarriers are completely dependent and determined by the scalar values of the these coefficients \TK{This fact complicates statistical analysis of the quadratic form of the channel}. 
% \\[\baselineskip]


==> sections/meta_prop_proof.tex <==
This section proves the statement given in XXX \TK{Insert ref to equation and possibly rewrite if some notation was introduced before}. We start by introducing some notation. The instantaneous capacity at location $\mbf{x}$, denoted by $C_{\mbf{x}}$, is given by \TK{Maybe put in some more derivations here (see outcommented appendix)}
\begin{align} 
    C_{\mbf{x}} = \sum_{j=0}^{N-1}\log_2\biggl(1 + \underbrace{\frac{P_{\text{tx}}P_L(d(\mbf{x}))\mbs{\psi}(\mbf{x})}{\sigma_n^2}}_{P_{\text{LS}}(\mbf{x})}\gamma_j(\mbf{x}) \biggr), \label{eq:capacity_proof}
\end{align}
where $P_{\text{LS}}(\mbf{x})$ is refereed to as the large scale fading factor, and 
\begin{align}
    \gamma_j(\mbf{x}) = \left| \sum_{k=1}^K \alpha_k(\mbf{x}) d_j(\tau_k(\mbf{x}))\right|^2 \label{eq:gamma1}
\end{align}
is proportional to the power of the frequency domain channel coefficients, where
\begin{align}
    \alpha_k(\mbf{x}) &= \e^{-\jmath \phi(d(\mbf{x}))} \ \text{for} \ k = 1  \\
    \alpha_k(\mbf{x}) &\sim \mathcal{CN}(0,\sigma^2(\tau_k(\mbf{x})) \ \text{for} \ 1 \leq k \leq K \label{eq:gamma3}
\end{align}
following Sec. \ref{subsec:chn_model}, where $\tau_k(\mbf{x})$ is the delay of path $k$ at location $\mbf{x}$. Next, the \gls{cdf} and inverse \gls{cdf} of $C_{\mbf{x}}$ is denoted $F_{\mbf{x}}$ and $F_{\mbf{x}}^{-1}$, respectively. 

Now consider the rate selection function $R_{\epsilon}(\hat{\mbf{x}}) = F_{\hat{\mbf{x}}}^{-1}(\epsilon)$ that selects the rate as the $\epsilon$-outage capacity at the estimated location $\hat{\mbf{x}}$. Given the true location of the \gls{ue} $\mbf{x}$, we are interested in characterizing the event that the outage probability exceeds $\epsilon$, hence
\begin{align} 
  P\left(R_{\epsilon}(\hat{\mbf{x}}) > C_{\mbf{x}} \cond \hat{\mbf{x}} \right) > \epsilon. \label{eq:meta_event}
\end{align}
for some $\epsilon \in (0,1)$. The statement to be proved is that, with the approximation $\tau_k(\hat{\mbf{x}}) = \tau_k(\mbf{x})$ for $k = 1,\dots, K$, the event in \eqref{eq:meta_event} coincides with the event that the large-scale fading factor at the estimated location exceeds the large-scale fading factor at the true location, i.e.,
\begin{align}
    \left(  P\left(R_{\epsilon}(\hat{\mbf{x}}) > C_{\mbf{x}} \cond \hat{\mbf{x}} \right) > \epsilon \right) \Leftrightarrow \left( P_{\text{LS}}(\hat{\mbf{x}}) > P_{\text{LS}}(\mbf{x}) \right) \label{eq:meta_result}
\end{align}
Two results are needed to prove \eqref{eq:meta_result}.
\begin{lemma} \label{lemma:lemma1}
Let $F_X$ and $F_Y$ be continuous \glspl{cdf} for the random variables $X$ and $Y$, respectively, both with range $R$. Then
\begin{align} \label{eq:lemma_statement}
F_X(x) < F_Y(x) \ \forall x \in R \Leftrightarrow F_X^{-1}(\epsilon) > F_Y^{-1}(\epsilon) \ \forall \epsilon \in (0,1),
\end{align}
where $F_X^{-1}$ and $F_Y^{-1}$ denote the inverse \glspl{cdf}, i.e., quantile functions. 
\end{lemma}
\begin{proof}
% Proof for inverse function inequality reversing: \href{https://math.stackexchange.com/questions/2329915/inequality-and-inverse-function}{link}
Assume that the left hand side of \eqref{eq:lemma_statement} is true and choose any $\epsilon \in (0,1)$. Since the \gls{cdf} $F_X$ is continuous and increasing, it is bijective, and the inverse $F_X^{-1}: (0,1) \to R$ exits (similarly for $F_Y)$. This means that, in particular, that there exists an $x \in R$ such that $F_Y(x) = \epsilon$. Choose this $x$ and note that $F_X(x) < F_Y(x)$. Additionally, since any \gls{cdf} is increasing, the inverse function will also be increasing and we can apply the inverse such that
\begin{align}
    F_X(x) < F_Y(x) \Rightarrow  F_X^{-1}(F_X(x)) < F_X^{-1}(F_Y(x)) 
\end{align}
However, since $F_X^{-1}(F_X(x)) = x = F_Y^{-1}(F_Y(x))$, we have
\begin{align}
     F_X(x) < F_Y(x) &\Rightarrow F_Y^{-1}(\epsilon) = F_Y^{-1}(F_Y(x)) < F_X^{-1}(F_Y(x)) = F_X^{-1}(\epsilon)
\end{align}
which proves $\Rightarrow$ in \eqref{eq:lemma_statement}. The proof for $\Leftarrow$ is completely equivalent. 
\end{proof}
\begin{lemma} \label{lemma:lemma2}
Let $F$ be a continuous \gls{cdf} for the random variables $X$ with range $R$ and consider the functions $h,\ g$ with domain $R$ and range $\mR$. Then we have the following
\begin{align}
    g(x)  < h(x) \ \forall x \in R \Leftrightarrow P(g(X) \leq x) > P(h(X) \leq x)  \ \forall x \in R \label{eq:lemma_statement2}
\end{align}
\end{lemma}
\begin{proof}
Start by assuming the left hand side of \eqref{eq:lemma_statement2} and choose some $x \in R$.  Define the set $I_g(x) = \{t \in R \cond g(t) \leq x \}$. Since $g(x) < h(x)$, we have that $I_h(x) = \{t \in R \cond h(t) \leq x \}$ is a subset of $I_g(x)$ so we have the following partition $I_g(x) = I_h(x) \cup \left( I_g(x) \setminus I_h(x)\right)$. The assertion then follows directly from the third axiom of probability:
\begin{align}
    P(g(X) \leq x) = P(X \in I_g(x)) &= P(X \in I_h(x)) + \underbrace{P(X \in I_g(x)\setminus I_h(x))}_{>0} \\
    &> P(X \in I_h(x)) = P(h(X) \leq x),
\end{align}
which proves $\Rightarrow$ in \eqref{eq:lemma_statement2}. 
\\[\baselineskip]
For the other direction, assume the right hand side of \eqref{eq:lemma_statement2} and chose $x \in R$ such that
\begin{align}
    P(g(X) \leq x) - P(h(X) \leq x) = \int_{I_g(x)} f(t) \ dt - \int_{I_h(x)} f(t) \ dt > 0, \label{eq:lemma_contradiction}
\end{align}
Now assume for contradiction that $g(x) \geq h(x)$. This implies that $I_g(x) \subseteq I_h(x)$ therefore
\begin{align}
    \int_{I_g(x)} f(t) \ dt \leq \int_{I_h(x)} f(t) \ dt,
\end{align}
which clearly contradicts \eqref{eq:lemma_contradiction}. Therefore we must have $g(x) < h(x)$. 
\end{proof}
Lemma \ref{lemma:lemma1} and \ref{lemma:lemma2} can now be used to prove \eqref{eq:meta_result}. We first rewrite the left hand side of \eqref{eq:meta_result}:
\begin{align}
     P\left(R_{\epsilon}(\hat{\mbf{x}}) > C_{\mbf{x}} \cond \hat{\mbf{x}} \right) = F_{\mbf{x}}(R_{\epsilon}(\hat{x})) > \epsilon \Leftrightarrow \\
    F^{-1}_{\mbf{x}}(F_{\mbf{x}}(R_{\epsilon}(\hat{x}))) = R_{\epsilon}(\hat{x}) = F_{\hat{\mbf{x}}}^{-1}(\epsilon) > F_{\mbf{x}}^{-1}(\epsilon) \label{eq:meta_result2}
\end{align}
Lemma \ref{lemma:lemma1} then tells that the event in \eqref{eq:meta_result2} coincides with the event that $F_{\hat{\mbf{x}}}(C_{\epsilon}) < F_{\mbf{x}}(C_{\epsilon})$ for  $C_{\epsilon} = F_{\hat{\mbf{x}}}^{-1}(\epsilon)$. We now define the random variable $\mbs{\gamma}_{\mbf{x}} = \begin{bmatrix} \gamma_1(\mbf{x}) & \dots & \gamma_K(\mbf{x}) \end{bmatrix}^\T$ given by \eqref{eq:gamma1}-\eqref{eq:gamma3}. According to \eqref{eq:capacity_proof}, the capacity can be considered as a function of $\mbs{\gamma}_{\mbf{x}}$ parameterized by the large scale fading factor $P_{\text{LS}}(\mbf{x})$, i.e., $C_{\mbf{x}} = C(\mbs{\gamma}_{\mbf{x}}; P_{\text{LS}}(\mbf{x}))$. Clearly, $C(\mbs{\gamma}_{\mbf{x}}; P_{\text{LS}}(\mbf{x})) < C(\mbs{\gamma}_{\mbf{x}};  P_{\text{LS}}(\hat{\mbf{x}}))$ if and only if $P_{\text{LS}}(\hat{\mbf{x}}) > P_{\text{LS}}(\mbf{x})$, so lemma \ref{lemma:lemma2} tells that
\begin{align}
P_{\mbs{\gamma}_{\mbf{x}}}\left[C(\mbs{\gamma}_{\mbf{x}}; P_{\text{LS}}(\hat{\mbf{x}})) < C_{\epsilon} \right] < P_{\mbs{\gamma}_{\mbf{x}}}\left[C(\mbs{\gamma}_{\mbf{x}}; P_{\text{LS}}(\mbf{x})) < C_{\epsilon} \right] \Leftrightarrow  P_{\text{LS}}(\hat{\mbf{x}}) > P_{\text{LS}}(\mbf{x})
\end{align}
We see that $F_{\mbf{x}}(C_{\epsilon}) = P_{\mbs{\gamma}_{\mbf{x}}}\left(C(\mbs{\gamma}_{\mbf{x}}; P_{\text{LS}}(\mbf{x})) < C_{\epsilon}\right)$, so it only remains to show that
\begin{align}
    F_{\hat{\mbf{x}}}(C_{\epsilon}) =  P_{\mbs{\gamma}_{\mbf{x}}}\left(C(\mbs{\gamma}_{\mbf{x}}; P_{\text{LS}}(\hat{\mbf{x}})) < C_{\epsilon}\right), \label{eq:same_dist}
\end{align}
which amounts to proving that $\mbs{\gamma}_{\hat{\mbf{x}}}$ and $\mbs{\gamma}_{\mbf{x}}$ follows the same distribution. With the earlier assumption that $\tau_k(\hat{\mbf{x}}) = \tau_k(\mbf{x})$ for $k = 1,\dots, K$, the two vectors are only different in $\alpha_1(\hat{\mbf{x}})$ and $\alpha_1(\mbf{x})$ that has different phase shift. However, we can easily see that
\begin{align}
    \gamma_j(\mbf{x}) = \left| \sum_{k=1}^K \alpha_k(\mbf{x}) d_j(\tau_k(\mbf{x}))\right|^2 = \left| \sum_{k=1}^K \alpha_k(\mbf{x})\e^{-\jmath(\phi(d(\hat{\mbf{x}})) - \phi(d(\mbf{x})))} d_j(\tau_k(\mbf{x}))\right|^2,
\end{align}
such that 
\begin{align}
    \alpha_1(\mbf{x})\e^{-\jmath(\phi(d(\hat{\mbf{x}})) - \phi(d(\mbf{x})))} = \e^{-\jmath\phi(d(\hat{\mbf{x}}))} = \alpha_1(\hat{\mbf{x}}),
\end{align}
and multiplying $\alpha_k(\mbf{x})$ with $\e^{-\jmath(\phi(d(\hat{\mbf{x}})) - \phi(d(\mbf{x})))}$ for $k > 1$ does not affect its distributing since it is a circular symmetric random variable. Thus $\gamma_j(\mbf{x})$ and  $\gamma_j(\hat{\mbf{x}})$ have the same distribution for $j = 0,\dots, N-1$, which proves \eqref{eq:same_dist}. 


